PDR: A Plug-and-Play Positional Decay Framework for LLM Pre-training Data Detection

Detecting pre-training data in Large Language Models (LLMs) is crucial for auditing data privacy and copyright compliance, yet it remains challenging in black-box, zero-shot settings where computational resources and training data are scarce. While existing likelihood-based methods have shown promise, they typically aggregate token-level scores using uniform weights, thereby neglecting the inherent information-theoretic dynamics of autoregressive generation. In this paper, we hypothesize and empirically validate that memorization signals are heavily skewed towards the high-entropy initial tokens, where model uncertainty is highest, and decay as context accumulates. To leverage this linguistic property, we introduce Positional Decay Reweighting (PDR), a training-free and plug-and-play framework. PDR explicitly reweights token-level scores to amplify distinct signals from early positions while suppressing noise from later ones. Extensive experiments show that PDR acts as a robust prior and can usually enhance a wide range of advanced methods across multiple benchmarks.

==> tables/camia_wiki.tex <==
\begin{table}[t]
\centering
\caption{\small{\bb{AUROC comparison on the WikiMIA benchmark. For each group of three methods,``w/ fitted LPDR" denotes applying LPDR with slope fitted on single test sample loss, while ``LPDR" uses a fixed default hyperparameter. The highest score per column is in \textbf{bold}. Our method's rows are highlighted in gray.}}}
\vspace{-5pt}
\label{tab:camia_wiki}
\renewcommand{\arraystretch}{1.3}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{llcccccccc}
\toprule
& & \multicolumn{2}{c}{\textbf{Pythia-2.8B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{Pythia-12B}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
\textbf{Len.} & \textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
\midrule

\multirow{12}{*}{32} 
&Loss & 61.37 & 61.57 & 63.83 & 64.07 & 65.44 & 65.60 & 63.55 & 63.75 \\
&w/fitted slope PDR & 61.42 & 61.60 & 63.79 & 64.06 & 65.33 & 65.60 & 63.52 & 63.75 \\
&\rowcolor{gray!15}w/LPDR & \textbf{61.73} & \textbf{61.83} & \textbf{63.97} & \textbf{64.20} & \textbf{65.45} & \textbf{65.70} & \textbf{63.71} & \textbf{63.91} \\
\cline{2-10}
&Ref & 61.34 & 61.17 & 63.57 & 63.52 & 65.12 & 64.86 & 63.34 & 63.19 \\
&w/fitted slope PDR & 61.22 & 61.11 & 63.44 & 63.31 & 64.95 & 64.69 & 63.20 & 63.04 \\
&\rowcolor{gray!15}w/LPDR & 61.34 & \textbf{61.18} & \textbf{63.55} & \textbf{63.47} & \textbf{65.09} & \textbf{64.90} & \textbf{63.33} & \textbf{63.18} \\
\cline{2-10}
&Min-$k$\% & 61.68 & 60.89 & 66.28 & 65.09 & 68.07 & 67.20 & 65.35 & 64.39 \\
&w/fitted slope PDR & 61.56 & 60.81 & 66.19 & 64.98 & 67.88 & 67.00 & 65.21 & 64.26 \\
&\rowcolor{gray!15}w/LPDR & \textbf{61.91} & \textbf{61.12} & \textbf{66.33} & \textbf{65.15} & \textbf{68.02} & 67.20 & \textbf{65.42} & \textbf{64.49} \\
\cline{2-10}
&Min-$k$\%++ & 63.97 & 61.33 & 70.27 & 67.56 & 72.24 & 69.40 & 68.83 & 66.10 \\
&w/fitted slope PDR & 64.08 & 61.48 & 70.37 & 67.70 & \textbf{72.32} & \textbf{69.56} & 68.92 & \textbf{66.24} \\
&\rowcolor{gray!15}w/LPDR & \textbf{64.74} & \textbf{61.66} & \textbf{70.85} & 67.74 & 72.26 & 69.36 & \textbf{69.28} & \textbf{66.25} \\
\midrule

\multirow{12}{*}{64} 
&Loss & 58.44 & 56.49 & 60.74 & 59.28 & 61.86 & 60.02 & 60.35 & 58.60 \\
&w/fitted slope PDR & 58.59 & 56.78 & 60.89 & 59.60 & 61.97 & 60.23 & 60.48 & 58.87 \\
&\rowcolor{gray!15}w/LPDR & \textbf{60.09} & \textbf{59.35} & \textbf{62.58} & \textbf{62.41} & \textbf{63.47} & \textbf{62.97} & \textbf{62.05} & \textbf{61.57} \\
\cline{2-10}
&Ref & 59.62 & 59.22 & 62.38 & 62.89 & 63.04 & 63.18 & 61.68 & 61.76 \\
&w/fitted slope PDR & 59.77 & 59.34 & 62.51 & 63.10 & 63.16 & 63.33 & 61.81 & 61.92 \\
&\rowcolor{gray!15}w/LPDR & \textbf{60.52} & \textbf{60.82} & \textbf{63.34} & \textbf{64.00} & \textbf{64.05} & \textbf{64.51} & \textbf{62.64} & \textbf{63.11} \\
\cline{2-10}
&Min-$k$\% & 61.20 & 56.68 & 64.97 & 61.07 & 66.50 & 62.49 & 64.22 & 60.08 \\
&w/fitted slope PDR & 61.39 & 57.03 & 65.19 & 61.40 & 66.69 & 62.79 & 64.42 & 60.41 \\
&\rowcolor{gray!15}w/LPDR & \textbf{63.26} & \textbf{61.59} & \textbf{66.67} & \textbf{65.07} & \textbf{67.94} & \textbf{66.08} & \textbf{65.95} & \textbf{64.25} \\
\cline{2-10}
&Min-$k$\%++ & 64.79 & 57.71 & 71.64 & 64.23 & 72.62 & 65.09 & 69.68 & 62.34 \\
&w/fitted slope PDR & 64.91 & 57.90 & 71.82 & 64.53 & 72.75 & 65.34 & 69.83 & 62.59 \\
&\rowcolor{gray!15}w/LPDR & \textbf{65.94} & \textbf{61.95} & \textbf{72.08} & \textbf{68.30} & \textbf{72.76} & \textbf{68.22} & \textbf{70.26} & \textbf{66.16} \\
\midrule

\multirow{12}{*}{128} 
&Loss & 62.81 & 62.31 & 65.08 & 64.66 & 65.77 & 65.40 & 64.55 & 64.12 \\
&w/fitted slope PDR & 62.85 & 62.32 & 65.07 & 64.82 & 65.81 & 65.47 & 64.58 & 64.20 \\
&\rowcolor{gray!15}w/LPDR & \textbf{63.12} & \textbf{63.97} & \textbf{65.64} & \textbf{66.63} & \textbf{66.25} & \textbf{67.01} & \textbf{65.00} & \textbf{65.87} \\
\cline{2-10}
&Ref & 59.57 & 59.54 & 63.27 & 62.92 & 63.93 & 63.91 & 62.26 & 62.12 \\
&w/fitted slope PDR & 59.84 & 59.80 & 63.47 & 63.29 & 64.02 & 64.06 & 62.44 & 62.38 \\
&\rowcolor{gray!15}w/LPDR & \textbf{61.42} & \textbf{62.56} & \textbf{65.07} & \textbf{65.90} & \textbf{65.05} & \textbf{66.16} & \textbf{63.85} & \textbf{64.87} \\
\cline{2-10}
&Min-$k$\% & 66.86 & 64.74 & 69.47 & 67.03 & 70.68 & 68.54 & 69.00 & 66.77 \\
&w/fitted slope PDR & \textbf{66.90} & \textbf{64.87} & 69.46 & 67.21 & \textbf{70.71} & \textbf{68.71} & 69.02 & 66.93 \\
&\rowcolor{gray!15}w/LPDR & 64.27 & 63.46 & \textbf{67.83} & \textbf{68.88} & 69.95 & 69.08 & 67.35 & \textbf{67.14} \\
\cline{2-10}
&Min-$k$\%++ & 66.32 & 62.67 & 69.77 & 65.88 & 71.83 & 67.70 & 69.31 & 65.42 \\
&w/fitted slope PDR & 66.40 & 62.75 & 69.82 & 66.09 & 71.97 & 67.81 & 69.40 & 65.55 \\
&\rowcolor{gray!15}w/LPDR & \textbf{66.80} & \textbf{65.77} & \textbf{72.39} & \textbf{72.20} & \textbf{73.50} & \textbf{72.19} & \textbf{70.90} & \textbf{70.05} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/camin_mimir.tex <==
\begin{table*}[htbp]
\caption{\bb{AUROC results on sub MIMIR datasets (DM Mathematics, Github, Pile CC). ``w/ fitted LPDR" denotes applying LPDR with slope fitted on single test sample loss, while ``LPDR" uses a fixed default hyperparameter. Results are bolded if they improve upon their respective baseline (Loss, Min-k\%, or Min-k++).}}
\label{tab:mimir_auc_subset}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt} % Adjust column spacing
\begin{tabular}{l ccccc ccccc ccccc}
\toprule
 & \multicolumn{5}{c}{\textbf{DM Mathematics}} & \multicolumn{5}{c}{\textbf{Github}} & \multicolumn{5}{c}{\textbf{Pile CC}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
\textbf{Method} & \textbf{160M} & \textbf{1.4B} & \textbf{2.8B} & \textbf{6.9B} & \textbf{12B} & \textbf{160M} & \textbf{1.4B} & \textbf{2.8B} & \textbf{6.9B} & \textbf{12B} & \textbf{160M} & \textbf{1.4B} & \textbf{2.8B} & \textbf{6.9B} & \textbf{12B} \\
\midrule
Loss & 48.84 & 48.53 & 48.36 & 48.47 & 48.47 & 65.75 & 69.82 & 71.29 & 73.01 & 73.99 & 49.56 & 50.01 & 50.09 & 50.69 & 51.07 \\
w/ fitted LPDR & 48.84 & 48.53 & 48.36 & 48.47 & 48.47 & 65.76 & 69.83 & 71.29 & 73.01 & 74.00 & 49.56 & 50.02 & 50.09 & 50.69 & 51.07 \\
LPDR & 48.72 & \textbf{48.60} & \textbf{48.40} & \textbf{48.51} & \textbf{48.57} & \textbf{66.04} & \textbf{70.04} & \textbf{71.50} & 72.99 & 73.94 & \textbf{49.91} & \textbf{50.43} & \textbf{50.49} & \textbf{51.05} & \textbf{51.39} \\
\midrule
Min-k\% & 49.27 & 49.29 & 49.10 & 49.16 & 49.21 & 65.65 & 69.96 & 71.44 & 73.26 & 74.24 & 50.10 & 50.47 & 50.46 & 51.20 & 51.48 \\
w/ fitted LPDR & 49.28 & 49.29 & 49.09 & 49.16 & 49.21 & 65.68 & 69.99 & 71.46 & 73.27 & 74.25 & 50.09 & 50.48 & 50.46 & 51.21 & 51.48 \\
LPDR & \textbf{49.52} & \textbf{49.70} & \textbf{49.25} & \textbf{49.47} & \textbf{49.54} & \textbf{65.93} & \textbf{70.20} & \textbf{71.66} & 73.16 & 74.09 & \textbf{50.24} & \textbf{51.00} & \textbf{51.07} & \textbf{51.65} & \textbf{51.94} \\
\midrule
Min-k\%++ & 50.12 & 50.17 & 50.21 & 50.52 & 50.42 & 64.66 & 69.63 & 70.88 & 72.80 & 74.18 & 49.67 & 50.04 & 49.78 & 51.19 & 51.75 \\
w/ fitted LPDR & 50.12 & 50.17 & 50.21 & 50.52 & 50.43 & 64.67 & 69.64 & 70.89 & 72.81 & 74.19 & 49.68 & 50.05 & 49.77 & 51.20 & 51.76\\
LPDR & 50.11 & \textbf{50.32} & 50.16 & 50.37 & \textbf{50.50} & 64.59 & 69.46 & 70.57 & 72.29 & 73.69 & 49.69 & \textbf{50.63} & \textbf{49.94} & \textbf{51.84} & \textbf{51.87} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/wiki_main.tex <==
\begin{table*}[t]
\centering
%\footnotesize
\caption{\small{AUROC results on WikiMIA benchmark \citep{mia_mink}. \textbf{w/ LPDR} utilizes our linear weights for reweighting. \textit{Ori.} and \textit{Para.} denote the original and paraphrased settings. {$^\dag$Neighbor results are from \citet{mia_mink_plus}.} For each method pair, the higher score is in \textbf{bold}. The performance gains of our method on the average results are highlighted in \color{purple}{purple}.}}
\vspace{-5pt}
\label{tab:wikimia_main}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.80\linewidth}{!}{
\begin{tabular}{llcccccccccccc}
\toprule
& & \multicolumn{2}{c}{\textbf{Mamba-1.4B}} & \multicolumn{2}{c}{\textbf{Pythia-6.9B}} & \multicolumn{2}{c}{\textbf{LLaMA-13B}} & \multicolumn{2}{c}{\textbf{GPT-NeoX-20B}} & \multicolumn{2}{c}{\textbf{OPT-66B}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}  
\textbf{Len.} & \textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
\midrule

\multirow{15}{*}{32} 
&Lowercase & 60.9 & 60.6 & 62.2 & 61.7 & 64.0 & 63.2 & 68.3 & 66.9 & 62.8 & 62.3 & 63.7 & 63.0 \\
&Zlib & 61.9 & 62.3 & 64.4 & 64.2 & 67.8 & 68.3 & 69.3 & 68.5 & 65.8 & 65.3 & 65.8 & 65.7 \\
&{$^\dag$Neighbor} & 64.1 & 63.6 & 65.8 & 65.5 & 65.8 & 65 & 70.2 & 68.3 & 68.2 & 66.7 & 66.8  & 65.8  \\ 
\cline{2-14}
&Loss & 61.0 & 61.3 & 63.8 & 64.1 & 67.5 & 68.0 & 69.1 & 68.6 & 65.6 & 65.3 & 65.4 & 65.5 \\
%&Loss + CAMIA & 61.1  & 61.5  & 63.8  & 64.1  & 67.5  & 68.0  & 68.9  & 68.4  & 65.5  & 65.1  & 65.4  & 65.4   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} (Ours) & \textbf{61.5} & \textbf{61.8} & \textbf{64.0} & \textbf{64.2} & \textbf{67.7} & \textbf{68.2} & 68.9 & 68.3 & 65.6 & 65.0 & \textbf{65.5}$^{\color{purple}{+0.1}}$ & 65.5 \\
\cline{2-14}
&Ref & 62.2 & 62.3 & 63.6 & 63.5 & 57.9 & 56.2 & 67.6 & 66.7 & 68.6 & 67.9 & 64.0 & 63.3 \\
%&Ref + CAMIA & 62.0  & 62.2  & 63.4  & 63.3  & 57.8  & 56.0  & 67.0  & 66.1  & 68.5  & 68.0  & 63.7  & 63.1   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & 62.2 & 62.3 & 63.5 & 63.5 & 57.8 & 56.1 & 67.4 & 66.6 & 68.6 & \textbf{68.0} & 63.9 & 63.3 \\
\cline{2-14}
&Min-$k$\% & 63.3 & 62.9 & 66.3 & 65.1 & 66.8 & 66.2 & 72.2 & 69.6 & 67.5 & 65.8 & 67.2 & 65.9 \\
%&Min-$k$\% + CAMIA & 63.3  & 62.9  & 66.3  & 65.1  & 66.8  & 66.2  & 72.2  & 69.6  & 67.5  & 65.8  & 67.2  & 65.9   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & \textbf{63.5} & \textbf{63.1} & 66.3 & 65.1 & 66.8 & 66.2 & 72.0 & 69.4 & \textbf{67.7} & 65.8 & \textbf{67.3}$^{\color{purple}{+0.1}}$ & 65.9 \\
\cline{2-14}
&Min-$k$\%++ & 66.4 & 65.7 & 70.3 & 67.6 & 84.4 & 82.7 & 75.1 & 69.7 & 69.7 & 67.0 & 73.2 & 70.5 \\
%&Min-$k$\%++ + CAMIA & 66.6  & 65.9  & 70.4  & 67.7  & 84.4  & 82.8  & 75.2  & 69.7  & 69.7  & 67.0  & 73.3  & 70.6   \\
&\rowcolor{gray!15}\textbf{w/ LPDR}  & \textbf{67.4} & \textbf{66.3} & \textbf{70.8} & \textbf{67.7} & \textbf{85.9} & \textbf{84.1} & \textbf{75.2} & 69.5 & \textbf{70.2} & \textbf{67.1} & \textbf{73.9}$^{\color{purple}{+0.7}}$ & \textbf{70.9}$^{\color{purple}{+0.4}}$ \\
\midrule
\multirow{11}{*}{64} 
&Lowercase & 57.0 & 57.0 & 58.2 & 57.7 & 62.0 & 61.0 & 66.3 & 65.6 & 61.1 & 60.0 & 60.9 & 60.3 \\
&Zlib & 60.4 & 59.1 & 62.6 & 61.6 & 65.3 & 65.3 & 68.1 & 66.5 & 63.9 & 62.2 & 64.1 & 62.9 \\
&{$^\dag$Neighbor} & 60.6 & 60.6 & 63.2 & 63.1 & 64.1 & 64.7 & 67.1 & 67.4 & 64.1 & 64.6 & 63.8  & 64.1  \\ 
\cline{2-14}
&Loss & 58.2 & 56.4 & 60.7 & 59.3 & 63.6 & 63.1 & 66.6 & 64.4 & 62.3 & 60.3 & 62.3 & 60.7 \\
%&Loss + CAMIA & 58.4  & 56.7  & 60.9  & 59.6  & 63.7  & 63.3  & 66.7  & 64.7  & 62.4  & 60.5  & 62.4  & 61.0   \\
&\rowcolor{gray!15}\textbf{w/ LPDR}  & \textbf{59.7} & \textbf{59.5} & \textbf{62.6} & \textbf{62.4} & \textbf{65.0} & \textbf{66.2} & \textbf{67.6} & \textbf{67.2} & \textbf{64.2} & \textbf{63.1} & \textbf{63.8}$^{\color{purple}{+1.5}}$ & \textbf{63.7}$^{\color{purple}{+3.0}}$ \\
\cline{2-14}
&Ref & 60.6 & 59.6 & 62.4 & 62.9 & 63.4 & 60.9 & 66.0 & 66.0 & 66.9 & 67.8 & 63.9 & 63.5 \\
%&Ref + CAMIA & 60.7  & 59.7  & 62.5  & 63.1  & 63.3  & 60.8  & 66.1  & 66.1  & 67.1  & 68.0  & 63.9  & 63.6   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & \textbf{61.1} & \textbf{60.8} & \textbf{63.3} & \textbf{64.0} & 59.8 & 57.9 & \textbf{66.8} & \textbf{67.2} & \textbf{68.2} & \textbf{69.1} & 63.9 & \textbf{63.8}$^{\color{purple}{+0.3}}$ \\
\cline{2-14}
&Min-$k$\% & 61.7 & 58.0 & 65.0 & 61.1 & 66.0 & 63.5 & 72.2 & 66.1 & 66.5 & 62.5 & 66.3 & 62.2 \\
%&Min-$k$\% + CAMIA & 62.0  & 58.3  & 65.2  & 61.4  & 66.1  & 63.7  & 72.3  & 66.4  & 66.7  & 62.8  & 66.5  & 62.5   \\
&\rowcolor{gray!15}\textbf{w/ LPDR}& \textbf{62.9} & \textbf{61.8} & \textbf{66.7} & \textbf{65.1} & \textbf{67.4} & \textbf{67.2} & 70.8 & \textbf{68.7} & \textbf{68.1} & \textbf{66.0} & \textbf{67.2}$^{\color{purple}{+0.9}}$ & \textbf{65.8}$^{\color{purple}{+3.6}}$ \\
\cline{2-14}
&Min-$k$\%++ & 67.2 & 62.2 & 71.6 & 64.2 & 84.3 & 78.8 & 76.5 & 66.2 & 69.8 & 63.3 & 73.9 & 66.9 \\
%&Min-$k$\%++ + CAMIA & 67.4  & 62.4  & 71.8  & 64.5  & 84.4  & 78.9  & 76.6  & 66.4  & 69.9  & 63.5  & 74.0  & 67.1   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & \textbf{68.2} & \textbf{65.5} & \textbf{72.1} & \textbf{68.3} & \textbf{87.2} & \textbf{84.3} & 76.4 & \textbf{68.2} & \textbf{70.1} & \textbf{66.6} & \textbf{74.8}$^{\color{purple}{+0.9}}$ & \textbf{70.6}$^{\color{purple}{+3.7}}$ \\
\midrule
\multirow{11}{*}{128} 
&Lowercase & 58.5 & 57.7 & 60.5 & 59.9 & 60.6 & 56.3 & 68.0 & 67.6 & 58.9 & 57.6 & 61.3 & 59.8 \\
&Zlib & 65.6 & 65.3 & 67.6 & 67.4 & 69.7 & 69.6 & 72.3 & 72.0 & 67.3 & 66.9 & 68.5 & 68.2 \\
&{$^\dag$Neighbor} & 64.8 & 62.6 & 67.5 & 64.3 & 68.3 & 64 & 71.6 & 69.6 & 67.7 & 63.4 & 68.0  & 64.8 \\ 
\cline{2-14}
&Loss & 63.3 & 62.7 & 65.1 & 64.7 & 67.8 & 67.2 & 70.7 & 69.7 & 65.5 & 64.5 & 66.5 & 65.7 \\
%&Loss + CAMIA & 63.3  & 62.8  & 65.1  & 64.8  & 67.7  & 67.2  & 70.8  & 69.8  & 65.5  & 64.5  & 66.5  & 65.8   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & \textbf{63.6} & \textbf{64.1} & \textbf{65.6} & \textbf{66.6} & \textbf{68.7} & \textbf{69.1} & 70.7 & \textbf{71.4} & \textbf{66.7} & \textbf{66.9} & \textbf{67.1}$^{\color{purple}{+0.6}}$ & \textbf{67.6}$^{\color{purple}{+1.9}}$ \\
\cline{2-14}
&Ref & 62.0 & 61.1 & 63.3 & 62.9 & 62.6 & 59.7 & 68.3 & 68.4 & 66.9 & 67.0 & 64.6 & 63.8 \\
%&Ref + CAMIA & 62.1  & 61.2  & 63.5  & 63.3  & 62.6  & 59.7  & 68.6  & 68.5  & 67.0  & 67.2  & 64.8  & 64.0   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & \textbf{64.1} & \textbf{64.6} & \textbf{65.1} & \textbf{65.9} & \textbf{64.9} & \textbf{61.7} & \textbf{69.5} & \textbf{70.2} & \textbf{68.6} & \textbf{69.5} & \textbf{66.4}$^{\color{purple}{+1.8}}$ & \textbf{66.4}$^{\color{purple}{+2.6}}$ \\
\cline{2-14}
&Min-$k$\% & 66.8 & 64.4 & 69.5 & 67.0 & 71.5 & 68.6 & 75.6 & 73.0 & 70.6 & 67.2 & 70.8 & 68.0 \\
%&Min-$k$\% + CAMIA & 66.9  & 64.5  & 69.5  & 67.2  & 71.6  & 68.8  & 75.8  & 73.1  & 70.7  & 67.4  & 70.9  & 68.2   \\
&\rowcolor{gray!15}\textbf{w/ LPDR}  & 65.5 & \textbf{65.8} & 67.8 & \textbf{68.9} & 71.2 & \textbf{71.0} & 74.5 & \textbf{75.2} & 70.6 & \textbf{69.9} & 69.9 & \textbf{70.2}$^{\color{purple}{+2.2}}$ \\
\cline{2-14}
&Min-$k$\%++ & 67.7 & 63.3 & 69.8 & 65.9 & 83.8 & 76.2 & 75.4 & 70.6 & 71.1 & 67.0 & 73.6 & 68.6 \\
%&Min-$k$\%++ + CAMIA & 67.8  & 63.5  & 69.8  & 66.1  & 83.9  & 76.4  & 75.5  & 70.7  & 71.3  & 67.2  & 73.7  & 68.8   \\
&\rowcolor{gray!15}\textbf{w/ LPDR} & \textbf{70.2} & \textbf{68.2} & \textbf{72.4} & \textbf{72.2} & \textbf{88.4} & \textbf{84.3} & \textbf{75.7} & \textbf{72.6} & \textbf{72.9} & \textbf{69.5} & \textbf{75.9}$^{\color{purple}{+2.3}}$ & \textbf{73.3}$^{\color{purple}{+4.7}}$ \\
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\end{table*}



==> tables/wiki_new_main.tex <==
\begin{table}[t]
\centering
\caption{\small{Summary of \textbf{average} AUROC (\%) results on WikiMIA benchmark across various models (Mamba-1.4B, Pythia-6.9B, LLaMA-13B, GPT-NeoX-20B, and OPT-66B). \textbf{w/ LPDR} utilizes our linear weights for reweighting. \textit{Ori.} and \textit{Para.} denote the original and paraphrased settings. {$^\dag$Neighbor results are from \citet{mia_mink_plus}.} For each method pair, the higher score is in \textbf{bold}. The performance gains of our method on the average results are highlighted in \color{purple}{purple}.}}
% \vspace{-5pt}
\label{tab:wikimia_summary}
\resizebox{0.98\linewidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Len. 32}} & \multicolumn{2}{c}{\textbf{Len. 64}} & \multicolumn{2}{c}{\textbf{Len. 128}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} \\
\midrule
Lowercase & 63.7 & 63.0 & 60.9 & 60.3 & 61.3 & 59.8 \\
Zlib & 65.8 & 65.7 & 64.1 & 62.9 & 68.5 & 68.2 \\
{$^\dag$Neighbor} & 66.8 & 65.8 & 63.8 & 64.1 & 68.0 & 64.8 \\
\cline{1-7}
Loss & 65.4 & 65.5 & 62.3 & 60.7 & 66.5 & 65.7 \\
%W/ LPDR (CAMIA slope) & 65.4  & 65.4& 62.4  & 61.0 & 66.5  & 65.8   \\
\rowcolor{gray!15}\textbf{w/ LPDR} (Ours) & \textbf{65.5}$^{\color{purple}{+0.1}}$ & 65.5 & \textbf{63.8}$^{\color{purple}{+1.5}}$ & \textbf{63.7}$^{\color{purple}{+3.0}}$ & \textbf{67.1}$^{\color{purple}{+0.6}}$ & \textbf{67.6}$^{\color{purple}{+1.9}}$ \\
\cline{1-7}
Ref & 64.0 & 63.3 & 63.9 & 63.5 & 64.6 & 63.8 \\
%W/ LPDR (CAMIA slope) & 63.7  & 63.1 & 63.9  & 63.6 & 64.8  & 64.0   \\
\rowcolor{gray!15}\textbf{w/ LPDR} (Ours)  & 63.9 & 63.3 & 63.9 & \textbf{63.8}$^{\color{purple}{+0.3}}$ & \textbf{66.4}$^{\color{purple}{+1.8}}$ & \textbf{66.4}$^{\color{purple}{+2.6}}$ \\
\cline{1-7}
Min-$k$\% & 67.2 & 65.9 & 66.3 & 62.2 & 70.8 & 68.0 \\
%W/ LPDR (CAMIA slope)& 67.2  & 65.9 & 66.5  & 62.5 & 70.9  & 68.2   \\
\rowcolor{gray!15}\textbf{w/ LPDR} (Ours)  & \textbf{67.3}$^{\color{purple}{+0.1}}$ & 65.9 & \textbf{67.2}$^{\color{purple}{+0.9}}$ & \textbf{65.8}$^{\color{purple}{+3.6}}$ & 69.9 & \textbf{70.2}$^{\color{purple}{+2.2}}$ \\
\cline{1-7}
Min-$k$\%++ & 73.2 & 70.5 & 73.9 & 66.9 & 73.6 & 68.6 \\
%W/ LPDR (CAMIA slope)& 73.3  & 70.6  & 74.0  & 67.1 & 73.7  & 68.8   \\
\rowcolor{gray!15}\textbf{w/ LPDR} (Ours)  & \textbf{73.9}$^{\color{purple}{+0.7}}$ & \textbf{70.9}$^{\color{purple}{+0.4}}$ & \textbf{74.8}$^{\color{purple}{+0.9}}$ & \textbf{70.6}$^{\color{purple}{+3.7}}$ & \textbf{75.9}$^{\color{purple}{+2.3}}$ & \textbf{73.3}$^{\color{purple}{+4.7}}$ \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table}
